MedHallTune: An Instruction-Tuning Benchmark for Mitigating Medical Hallucination in Vision-Language Models

The increasing use of vision-language models (VLMs) in healthcare applications presents great challenges related to hallucinations, in which the models may generate seemingly plausible results that are in fact incorrect. Such hallucinations can jeopardize clinical decision making, potentially harming the diagnosis and treatments. In this work, we propose MedHallTune, a large-scale benchmark designed specifically to evaluate and mitigate hallucinations in medical VLMs. Comprising over 100,000 images and 1,000,000 instruction pairs, MedHallTune includes both hallucination and non-hallucination samples, each with ground-truth annotations. We conduct a comprehensive evaluation of current medical and general VLMs using MedHallTune, assessing their performance across key metrics, including clinical accuracy, relevance, detail level, and risk level. The experimental results show that fine-tuning with MedHallTune successfully improves the ability of several existing models to manage hallucinations and boost their zero-shot performance on downstream visual-question-answering (VQA) tasks, making them more reliable for practical medical applications. Our work contributes to the development of more trustworthy VLMs. Codes and dataset will be available at \href{https://github.com/russellyq/MedHallTune}{MedHallTune}.

==> tabels/backup.tex <==
\begin{table}[]
\begin{tabular}{lcccccccccccc}
\hline
Method             & P-Acc & N-Acc & P-Rel & N-Rel & P-Detail & N-Detail & P-Risk & N-Risk & P-BScore & N-BScore & P-MScore & N-MScore \\ \hline
GPT-4o             & 6.52  & 5.01  & 7.08  & 5.66  & 6.44     & 5.43     & 7.68   & 6.23   & 0.88     & 0.87     & 0.34     & 0.26     \\
GPT-5              & 6.48  & 5.75  & 7.02  & 6.49  & 6.44     & 6.31     & 7.98   & 7.15   & 0.86     & 0.84     & 0.21     & 0.19     \\
o3                 & 6.32  & 5.77  & 6.81  & 6.44  & 6.00     & 5.99     & 7.71   & 7.10   & 0.89     & 0.86     & 0.25     & 0.21     \\
Grok-4             & 6.67  & 5.36  & 7.21  & 5.91  & 6.54     & 5.81     & 7.92   & 6.72   & 0.90     & 0.85     & 0.27     & 0.23     \\
Gemini-2.5         & 6.51  & 5.28  & 6.98  & 5.81  & 6.15     & 5.50     & 8.00   & 6.60   & 0.88     & 0.87     & 0.33     & 0.26     \\ \hline
MiniGPT-4          & 4.46  & 3.24  & 4.71  & 3.48  & 4.71     & 4.22     & 5.91   & 4.48   & 0.85     & 0.86     & 0.23     & 0.23     \\
Janus-Pro-7B       & 6.17  & 4.12  & 6.73  & 4.51  & 5.53     & 4.61     & 7.43   & 5.21   & 0.91     & 0.89     & 0.39     & 0.22     \\
mPLUG-Owl2-7B      & 5.97  & 3.94  & 6.43  & 4.29  & 5.72     & 4.71     & 7.16   & 5.05   & 0.90     & 0.88     & 0.36     & 0.27     \\
LLaVA-Critic-R1-7B & 6.14  & 4.27  & 6.56  & 4.81  & 6.11     & 5.01     & 7.64   & 5.61   & 0.86     & 0.86     & 0.25     & 0.28     \\
LLaVA-OneVision-8B & 6.50  & 4.72  & 7.04  & 5.13  & 5.46     & 4.78     & 7.05   & 5.80   & 0.91     & 0.88     & 0.38     & 0.19     \\
OpenMMReasoner-7B  & 6.29  & 4.99  & 6.75  & 5.22  & 5.62     & 5.01     & 7.61   & 5.24   & 0.86     & 0.86     & 0.28     & 0.25     \\
Qwen-VL-Chat       & 5.95  & 4.21  & 6.45  & 4.57  & 5.54     & 4.60     & 7.17   & 5.42   & 0.90     & 0.88     & 0.35     & 0.19     \\
Qwen2.5-VL-7B      & 6.12  & 4.28  & 6.53  & 4.82  & 6.11     & 4.65     & 7.54   & 5.64   & 0.85     & 0.86     & 0.25     & 0.23     \\
Qwen3-VL-8B        & 6.28  & 4.86  & 6.68  & 5.11  & 6.79     & 4.86     & 7.80   & 5.60   & 0.83     & 0.83     & 0.21     & 0.25     \\
InternVL-v1.5-4B   & 6.02  & 4.25  & 6.59  & 4.68  & 5.29     & 4.56     & 7.28   & 5.31   & 0.90     & 0.87     & 0.30     & 0.23     \\
InternVL2.5-8B     & 6.03  & 4.82  & 6.43  & 5.27  & 5.28     & 4.90     & 7.59   & 5.14   & 0.90     & 0.87     & 0.33     & 0.20     \\
InternVL3-8B       & 6.23  & 4.64  & 6.74  & 5.05  & 5.16     & 4.67     & 7.63   & 5.39   & 0.88     & 0.87     & 0.24     & 0.14    
\end{tabular}
\end{table}
